Low-Precision Quantization for Efficient Nearest Neighbor Search

Fast k-Nearest Neighbor search over real-valued vector spaces (KNN) is an important algorithmic task for information retrieval and recommendation systems. We present a method for using reduced precision to represent vectors through quantized integer values, enabling both a reduction in the memory overhead of indexing these vectors and faster distance computations at query time. While most traditional quantization techniques focus on minimizing the reconstruction error between a point and its uncompressed counterpart, we focus instead on preserving the behavior of the underlying distance metric. Furthermore, our quantization approach is applied at the implementation level and can be combined with existing KNN algorithms. Our experiments on both open source and proprietary datasets across multiple popular KNN frameworks validate that quantized distance metrics can reduce memory by 60% and improve query throughput by 30%, while incurring only a 2% reduction in recall.

==> tex/limitations.tex <==
\section{Limitations}
\label{sec:limitations}

\todo{No room for this in a workshop paper}

Compression schemes work best when they result in a bit-width encoding which is a power of two. Densely-packed data with this property can be aligned to a target architecture’s native word boundaries, and machine instructions which target data in this configuration can be many times faster than the alternative. While there is value in knowing that we can reduce the precision of vectors to 6-bits without sacrificing precision, the performance impact of dense-packing those values between 8-bit word boundaries would be quite significant. As a result, even if we were to choose an encoding below 8-bits, performance considerations would force us to align the values to the smallest native integer word available on commodity hardware (typically {\tt int8}).

Compression schemes also need to preserve the overall distribution of the original data. The shape of each dimension is how the distance calculation is able consistently group several vectors as close neighbors even with low precision. 


==> tex/notions.tex <==
\section{Intuitions and Notions of Quantization}
\label{sec:motivation}

\todo{This entire section becomes one paragraph in the intro.}

\begin{comment}
\subsection{Low Precision Recall}

Figure~\ref{fig:recall} plots compares recall for integer bit-width encodings against a full 64-bit floating-point implementation of exact-KNN. The results are computed for varying values of $K$ on a hold-out test set of 1,000 queries. We define recall using the standard formula which counts the number of results $n$, which appear in both the reference result set and the low-precision result set. Bit-width encodings between 6 and 8 introduced less than 3\% precision loss for $K>5$ relative to uncompressed data. 
5- and 6-bit encodings introduced a losses between 10 and 20\%, rates which may be usable depending on the application. The remaining encoding schemes, introduced non-trivial errors.

While our integer encoding scheme works empirically, it is good to consider why this should be the case. Intuitively, our goal is preserve the value of the full-precision KNN computation. For a dataset of $M$ vectors and a fixed value of $K$, our encoding scheme should allows for at least $\frac{M}{K}$ unique values of the distance metric. If we were incapable of representing this many distances, then we would be incapable of distinguishing the distance between a query, the top $K$ vectors, and the rest of the dataset. Thus, for $M=3$M and $K=200$, a compression scheme should be capable of representing at least $30,000$ unique distances. Consider:
\begin{itemize}
    \item A $B$-bit encoding can represent $2^B$ unique feature values between $-(2^{B-1})$ and $2^{B-1}$. The special case of $B=1$ can represent two: -1 and 1.
    \item The product of two any two $B$-bit feature can be no more than one of ${2^B}^2 = 2^{2B}$ values. In practice, this value will be smaller due to aliasing: the pairs $(2,-3)$ and $(-2,3)$ have the same product.
    \item The number of unique dot products for two B-bit d-dimensional vectors can be no more than $2^{2B} \times d$. Intuitively, the largest sum we can obtain is one where each pair of elements multiplies to ${2^{B-1}}^2$, and the smallest we can obtain is where each pair multiplies to $-({2^{B-1}}^2)$. All other unique dot products fall somewhere in this range.
\end{itemize}

Figure~\ref{fig:counting} compares the number of unique point-wise, and dot-products for bit-width encodings between 1 and 6. For 7 and 8, we approximate the results using the observation that as bit-width grows, the true number of unique dot-product values trends towards $\frac{1}{2}$ of the upper bound described above. The final column in the table shows the number of unique dot-product distances as a percentage of $30,000$. The results align well with Figure~\ref{fig:recall}. Bit-width encodings between 6 and 8 produce many times more unique distances than what are required to distinguish the top 200 nearest neighbors. Encodings between 4 and 5 are a small constant factor away from the critical value, and encodings between 1 and 3 result in far too few unique distances and an unacceptable loss of precision.

\begin{figure}[t]
\centering
\begin{tabular}{rrrrr}
Bits & Range & Point Products & Dot Products & Percent of 30k \\
\hline
1&	$(-1,1)$&	2&	257&	0.008\\
2&	$(-2,1)$& 	6&	1,536&	0.051\\
3&	$(-4,3)$&	18&	7,160&	0.238\\
4&	$(-8,7)$&	60&	30,682&	1.02\\
5&	$(-16,15)$&	194&	126,842&	4.22\\
6&	$(-32,31)$&	708&	515,669&	17.2\\
7&	$(-64,63)$&	2,526&	$\approx2,097,152$&	~69.9\\
8&	$(-128,127)$& 9,390&	$\approx8,388,608$&	~279\\
\end{tabular}
\caption{Comparison of bit-width encoding schemes and the number of unique values the cosine similarity distance metric can return over that domain. Comparing this value to the ratio of dataset size to $K$ is a good predictor of recall.}
\label{fig:counting}
\end{figure}
\end{comment}

\subsection{{\tt float32} to {\tt int8} (could be in a different section)}
When compressing from {\tt float32} to {\tt int8}, we can simply look at it as
reducing from $3.4\times 10^{38}$ bins to $256$ bins. However, this means all
possible values for {\tt float32} is used, which is likely not the case. In
many situations, only a small range of numbers will be used. In our
experiments, the data ranges only from around $\pm 0.13$, which is only around
1.3 million bins, which may differ in each dimension. Because there are so many
values that can be mapped to each {\tt int8} bin, it is important to maintain
the shape of each dimension after compression, as the distance calculation is
very dependent on the distributions. 

\subsection{Case Study}

\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{0.45\textwidth}
        \hspace*{-.6cm}  
        \includegraphics[scale=0.48]{fig/dist.pdf}
        \caption{Distribution of values in a O(100M) vector production dataset. The values fall in a very now band of what is representable using floating-point precision.}
        \label{fig:dist}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.45\textwidth}
        \hspace*{-.6cm}  
        \includegraphics[scale=0.48]{fig/recall.pdf}
        \caption{Recall on a production dataset as a function of $K$ and compression rate. $90\%$ recall can be achieved with as few as 5-integer bits per value.}
        \label{fig:recall}
    \end{minipage}
\end{figure*}

We now present a case study of a hundred-million-scale production data set maintained by a large e-commerce company. Our goal is to develop intuitions which will guide the development of the formalism in the following section. The dataset consists of 100 million vectors, each of which comprise 256 feature values. The vectors are normalized to the standard unit ball, and cosine similarity is used as a distance metric.  

% \subsection{Low Precision Vector Quantization}

Clearly, the use of floating-point primitives as a representational format for this dataset is over-provisioned. {\tt float64}, {\tt float32}, and {\tt float16} can represent values with magnitudes in the ranges ($2^{-1024}$,$2^{1023}$), ($2^{-128}$,$2^{127}$), and ($2^{-16}$,$2^{15}$), respectively. However, as there is neither a standard for lower-precision floating-point primitives, nor commodity hardware support for operations on such primitives, we must look elsewhere for an alternative representational format.

